Fair Clustering Using Antidote Data

Clustering algorithms are widely utilized for many modern data science applications. This motivates the need to make outputs of clustering algorithms fair. Traditionally, new fair algorithmic variants to clustering algorithms are developed for specific notions of fairness. However, depending on the application context, different definitions of fairness might need to be employed. As a result, new algorithms and analysis need to be proposed for each combination of clustering algorithm and fairness definition. Additionally, each new algorithm would need to be reimplemented for deployment in a real-world system. Hence, we propose an alternate approach to group-level fairness in center-based clustering inspired by research on data poisoning attacks. We seek to augment the original dataset with a small number of data points, called antidote data. When clustering is undertaken on this new dataset, the output is fair, for the chosen clustering algorithm and fairness definition. We formulate this as a general bi-level optimization problem which can accommodate any center-based clustering algorithms and fairness notions. We then categorize approaches for solving this bi-level optimization for two different problem settings. Extensive experiments on different clustering algorithms and fairness notions show that our algorithms can achieve desired levels of fairness on many real-world datasets with a very small percentage of antidote data added. We also find that our algorithms achieve lower fairness costs and competitive clustering performance compared to other state-of-the-art fair clustering algorithms.

==> discussion.tex <==
\looseness-1 A major limitation of our work is running time. We present empirical results in the appendix (Section E). While not prohibitively slow, in comparison to fair clustering algorithms, Algorithm 1 is generally slower and requires careful parameterization for convergence. Similar limitations hold for the other algorithms. However, we believe that despite these shortcomings, our paper opens up an important alternative direction for future research in fair clustering, as our experiments also demonstrate. 

%-- for example, the first work on fair clustering \citep{chierichetti2017fair} did not scale well with data and could only accommodate 2 protected groups, and yet lead to many papers with subsequent improvements.
%%, with Algorithm 3 incurring the extra overhead of the process used to find fair centers.

==> scratch.tex <==
%%SECTION 4.1
\iffalse
\begin{algorithm}
\caption{Proposed Algorithm for General $\mathcal{C}$ and $\mathcal{F}$}\label{sre}
\textbf{Input:} $U, \mathcal{C}, \mathcal{F}, \mathcal{A}, V_s, n', \xi$\\
\textbf{Output:} $V$
 \begin{algorithmic}[1]
 \Function{$f$}{$U, V, \mathcal{C}, \mathcal{F}$}
    \State $\mu \leftarrow \mathcal{C}(U \cup V)$
    \State \textbf{return} $\mathcal{F}(\mu, U)$
 \EndFunction
 \Statex
 \While{$\mathcal{F}(\mu, U) > \alpha$}
 \State \textbf{initialize} $V$ randomly with $|V| = V_s$
 \State \textbf{optimize} $V$ using \texttt{SRE}($n', f(U, V, \mathcal{C}, \mathcal{F}), \mathcal{A}$) 
 \State \textbf{obtain} optimized $V$ and $\mathcal{F}(\mu, U)$ as output from \texttt{SRE} and $\mathcal{A}$
 \State \textbf{if} $\mathcal{F}(\mu, U) \leq \alpha$ \textbf{return} $V$ \textbf{else} $V_s \leftarrow V_s + \xi$
 \EndWhile
 \end{algorithmic}
\end{algorithm}
\fi

Due to the blackbox and general nature of this setting, it is hard to give theoretical results about convergence and optimality. However, in the following subsections, when we can make some restrictive assumptions about $\mathcal{C}$ and $\mathcal{F}$, we provide more theoretical justification for our approaches. Furthermore, in our experiments on real-world data and in practice, we find that we can achieve improved fairness using Algorithm \ref{sre} with relative ease.


%%%SECTION 4.2

In this setting, we assume that both $\mathcal{C}$ and $\mathcal{F}$ are convex functions. This allows us to model the bi-level problem P1 much more easily since we know that a global optimum exists for the lower-level clustering problem. We now describe the standard approach for reducing the bi-level problem to a single-level optimization problem which is easier to solve:
\begin{enumerate}
    \item Derive the Karush-Kuhn-Tucker (KKT) conditions for the lower-level problem in P1.
    \item Replace the lower-level problem with the KKT conditions as constraints for the upper-level problem.
    \item Solving the obtained single-level problem is equivalent to solving P1.
\end{enumerate}

To extrapolate on the above approach for this setting, we can consider a convex clustering objective $\mathcal{C}$ and a convex $\mathcal{F}$. We can see that the social fairness cost $ \mathcal{F}_{\textrm{social}}$ is convex so we will consider that as our fairness notion. For $\mathcal{C}$, we consider a convex clustering objective called sum-of-norms (SON) clustering \citep{son, son-hier, son-kme, jiang2020identifying}. The SON clustering objective is strictly convex, and has been shown to be a relaxation for both k-means \citep{son-kme} and hierarchical clustering \citep{son-hier} approaches. The clustering objective is as follows:
\begin{equation}\tag{P2}
    \mathcal{C}_{\textrm{SON}}(U) \coloneqq \mu = \argmin_{\mu' \in \mathbb{R}^{n \times d}} \frac{1}{2}\sum_{j=1}^n||U_j - \mu_j'||^2 + \lambda\sum_{i<j}||\mu_i' - \mu_j'||
\end{equation}

Here the first term refers to a minimization between points and centers, and the second is a regularization term controlled by $\lambda$ to avoid trivial solutions. Moreover, we can have some $k$ centers by appropriate selection of $\lambda$ but due to how the objective is structured, we let $\mu \in \mathbb{R}^{n \times d}$. That is, some points will have the same centers and there will only be $k$ unique centers in $\mu$. 

We also borrow some ideas from \citep{Sun2021ConvexCM} which will allow us to derive the KKT conditions. Firstly, it is easier to model the regularization term if we create an ordering of all $(\mu_i, \mu_j)$ pairs that follow that $i < j$. Also, we can let each of the $n$ centers $\mu_i$ be a node in a graph $G$. Then, the ordering we have created, essentially enumerates the list of edges $E$ for the graph $G$. We denote this ordering as $O$ where we will have $|E| = |O|$. We also denote the node-arc-incidence matrix \citep{node-arc} for $(G, E)$ as $J \in \mathbb{R}^{n \times |O|}$. Using these, we can rewrite the objective in P2 as (where $\eta \in \mathbb{R}^{d \times |O|}$ is an auxiliary parameter):

\begin{equation}\tag{P3}
 \begin{aligned}
\min_{\mu, \eta} \quad & \frac{1}{2} ||\mu - U||^2 + \lambda \sum_{i \in O}||\eta^i||\\
\textrm{s.t.} \quad &  \mu^{T}J - \eta = 0\\
\end{aligned}   
\end{equation}

We can now also define the dual of problem P3 using the parameters $\theta \in \mathbb{R}^{d \times n}$ and $\zeta \in \mathbb{R}^{d \times |O|}$:


\begin{equation}\tag{P4}
 \begin{aligned}
\max_{\theta, \zeta} \quad &  \langle U^T, \theta \rangle - \frac{1}{2}||\theta||^2\\
\textrm{s.t.} \quad &  \zeta J^T - \theta = 0\\
& ||\zeta_i|| \leq \lambda, \forall i \in O\\
\end{aligned}   
\end{equation}


The KKT conditions for P3 and P4 are as follows (where prox(.) refers to the proximal operator of the Euclidean norm):
\begin{equation}\tag{KKT}
\begin{aligned}
    & \theta + \mu - U = 0\\
    & \eta - \textrm{prox}(\eta + \zeta) = 0\\
     & \mu^{T}J - \eta = 0\\
     & \zeta J^T - \theta = 0\\
\end{aligned} 
\end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this setting, we assume that both $\mathcal{C}$ and $\mathcal{F}$ are convex functions. We derive a negative result regarding the use of antidote data in this case, and for completeness, provide algorithms that compute fair centers as well. In particular, no other work has looked at convex clustering objectives from a fairness perspective, so ours is also the first work to do so. For any arbitrary $\mathcal{C}$ and $\mathcal{F}$ that are convex in $\mu$ we find that we can solve the bi-level problem and obtain the global optima without adding any antidote data. This is summarized in the following result:

\begin{claim}\label{no_antidote}
\textit{If $\mu^*$ is the optimal set of fair centers for problem \ref{p1} where both the clustering objective $\mathcal{C}$ and fairness cost $\mathcal{F}$ are convex functions, then an algorithm exists that obtains $\mu^*$ with $V$ set to $\emptyset$.}
\end{claim}

Effectively, if we consider solving problem \ref{p1} with $V \leftarrow \emptyset$, it reduces to solving problem \ref{p1.r} with $V \leftarrow \emptyset$. If $\mathcal{C}$ and $\mathcal{F}$ are convex in $\mu$ then Claim \ref{no_antidote} holds, and we can obtain the optimal center set $\mu^*$. If $\mathcal{F}(\mu^*, U) \leq \alpha$ then problem \ref{p1} is infeasible, otherwise we have found the optimal solution. We now discuss approaches towards solving the aforementioned problem.

\textbf{A standard first approach.} A simple approach towards solving the problem is to perform a single-level reduction from the bi-level form. This can be done by replacing the lower-level problem with its Karush-Kuhn-Tucker optimality conditions as constraints for the upper-level problem \citep{sinha2017review}. However, the obtained single-level optimization problem can now be non-convex, since the complementarity KKT condition can be non-convex. One would have to employ a non-convex solver for this problem, and in doing so, only locally optimal solutions are guaranteed. We thus give an improved approach based on bi-level subgradient descent, with strong theoretical guarantees of convergence to the globally optimal solution. 

\textbf{Subgradient descent based approach.} Since both the upper-level and lower-level problems are convex, we can utilize the subgradients of each function to optimize the overall bi-level problem. We first present our simple algorithm as Algorithm 

\begin{algorithm}
\caption{Proposed Algorithm for Convex $\mathcal{C}$ and $\mathcal{F}$}\label{cvx}
\textbf{Input:} \\
\textbf{Output:} 
 \begin{algorithmic}[1]
 \end{algorithmic}
\end{algorithm}
